Measuring Fairness in Financial Transaction Machine Learning Models

Mastercard, a global leader in financial services, develops and deploys machine learning models aimed at optimizing card usage and preventing attrition through advanced predictive models. These models use aggregated and anonymized card usage patterns, including cross-border transactions and industry-specific spending, to tailor bank offerings and maximize revenue opportunities. Mastercard has established an AI Governance program, based on its Data and Tech Responsibility Principles, to evaluate any built and bought AI for efficacy, fairness, and transparency. As part of this effort, Mastercard has sought expertise from the Turing Institute through a Data Study Group to better assess fairness in more complex AI/ML models. The Data Study Group challenge lies in defining, measuring, and mitigating fairness in these predictions, which can be complex due to the various interpretations of fairness, gaps in the research literature, and ML-operations challenges.

==> figures/process.tex <==
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!30]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!30]
\tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=gray!30]
\tikzstyle{arrow} = [thick,->,>=stealth]


\begin{tikzpicture}[node distance=2.5cm and 4cm]

\node (owner) [startstop] {Owner Trained Model};
\node (outsource) [process, below of=owner] {Outsource Predictions to Bank};
\node (use) [process, below of=outsource] {Use Predictions to Make Decisions};
\node (decision) [decision, below of=use, yshift=-1cm] {Decisions};
\node (good) [process, below right of=decision, xshift=2.5cm, yshift=-1cm] {Take Good Decisions};
\node (bad) [process, below left of=decision, xshift=-2.5cm, yshift=-1cm] {Take Wrong Decisions};
\node (fair) [startstop, right of=good, xshift=3cm] {Fair Treatments};
\node (harm) [startstop, right of=bad, xshift=3cm] {Allocation of Harms \& Discrimination};

\draw [arrow] (owner) -- (outsource);
\draw [arrow] (outsource) -- (use);
\draw [arrow] (use) -- (decision);
\draw [arrow] (decision) -- node[anchor=south] {yes} (good);
\draw [arrow] (decision) -- node[anchor=south] {no} (bad);
\draw [arrow] (good) -- (fair);
\draw [arrow] (bad) -- (harm);

\end{tikzpicture}


  

==> sections/definition_fairness.tex <==
\section{Defining Fairness}\label{sec:defining}
\subsection{Defining Fairness in Financial Transactions}


In our study, fairness is defined not in the typical context of resource allocation but rather as the quality of service provided to customers. While many studies understand fairness in terms of resource distribution across various sectors such as education and healthcare, our focus is on ensuring that all customers receive the same level of service and satisfaction.

Unlike other banking products, where historical biases across gender and race are well-understood and documented, measuring fairness within predictive models requires a different approach. For example, in mortgage lending, disparities in approval rates between different demographic groups have been extensively studied and legislated against through acts like the Equal Credit Opportunity Act in the UK and The Federal Equal Credit Opportunity Act in the US. These laws ensure that lending practices do not unfairly discriminate against individuals based on race, gender, or other protected characteristics. In contrast, predicting future purchase behavior requires a different approach:

\emph{How can we decide whether a predictive model is fair when the dataset shows that certain groups of people buy more specific products, such as makeup?}

If our data indicates that women buy more makeup and we build a model for targeted ads, it might end up recommending makeup primarily to women. 


\emph{Is this bias, or is it simply reflecting reality?}

The term "bias" fails to capture the complexity of the issue, as AI recommendations reflect existing consumption patterns rather than inherent bias. However, AI should not just reproduce societal norms but promote inclusivity. By orienting AI towards emerging trends, such as recommending makeup to men and non-binary individuals, we can prevent it from replicating the status quo and instead create opportunities for broader consumption patterns. This proactive approach ensures minority groups are not excluded, harnessing AI to contribute positively to social change. Integrating fairness into AI not only attracts and retains customers but also mitigates regulatory and reputational risks, leading to sustainable performance and increased brand value.
 


\subsection{Selecting a Measure of Fairness}


\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{\textbf{Confusion Matrix}} \\ \hline
        \rowcolor{gray!20}
        & \textbf{Predicted Positive} & \textbf{Predicted Negative} \\ \hline
        \textbf{Actual Positive} & 
        \cellcolor{green!30} True Positive (TP) & 
        \cellcolor{red!30} False Negative (FN) \\ \hline
        \textbf{Actual Negative} & 
        \cellcolor{yellow!30} False Positive (FP) & 
        \cellcolor{blue!30} True Negative (TN) \\ \hline
    \end{tabular}
    \caption{Confusion Matrix Visualization of True Positives, False Positives, True Negatives, and False Negatives}
    \label{tab:confusion_matrix}
\end{table}

In society, privileged groups often receive preferential treatment and access to higher-quality services, even when they may not fully qualify for them. This results in financial advantages and better opportunities for these individuals. Conversely, underprivileged groups frequently face unfair treatment, being denied advantageous services or lacking suitable options that address their specific needs. Systemic biases disproportionately favour privileged groups, leading to decision-making processes that overlook the diverse needs of underprivileged communities. To address these issues, it is essential to carefully select and balance measures of fairness in predictive models to avoid perpetuating existing societal biases.

When evaluating fairness in financial transaction predictive models, differences in errors can increase inequalities. These errors include false positives and false negatives, each with significant implications.

\subsubsection{Types of Errors and Their Impact}

\textbf{False Positives (FP):} False positives occur when a model incorrectly predicts a positive outcome for an individual who does not genuinely qualify for it. In financial transactions, false positives can perpetuate privilege by granting benefits or advantages, such as credit approval or favourable interest rates, to individuals who may not actually deserve them. This misallocation can lead to an unfair concentration of resources and opportunities within already privileged groups.

\textbf{False Negatives (FN):} False negatives occur when a model fails to identify a positive outcome for an individual who genuinely qualifies for it. False negatives can perpetuate underprivileged by unjustly denying opportunities or resources, such as loan approvals or lower interest rates, to individuals who are entitled to them. This misallocation can further disadvantage already underprivileged groups, exacerbating existing inequalities.

\subsubsection{Examples in Financial Services}

To illustrate these concepts, consider the following outcomes in the context of offering financial services by a company like Mastercard:

\textbf{True Positive (TP):} A creditworthy individual is correctly offered a credit card or loan product that aligns with their financial profile and needs.

\textbf{False Negative (FN):} An individual from an underrepresented group with good creditworthiness is incorrectly denied a suitable credit product due to bias in the predictive model's training data or decision logic. This could happen if the model fails to accurately assess the financial profiles of certain demographic groups. Additionally, a false negative can occur if the company does not offer tailored financial products that meet the specific needs of underprivileged groups. For example, not offering small business loans designed for entrepreneurs from underrepresented communities could result in qualified applicants being denied suitable financing options.

\textbf{False Positive (FP):} An unqualified applicant is erroneously approved for a premium loan or a more advantageous financial product. While this decision by the predictive model is incorrect, it may temporarily improve the individual's financial situation undeservedly, as they do not genuinely meet the criteria for the product. For example, an individual with a poor credit history might mistakenly receive a premium credit card or loan product, potentially leading to financial difficulties.

\textbf{True Negative (TN):} An individual with a low credit score or insufficient income is correctly denied a credit product that they do not meet the qualifications for at their current financial standing.



\subsection{Stakeholders in Financial Transactions}

A significant disparity exists between users of predictive models (e.g., banks) and those impacted by these predictions (e.g., cardholders). Mastercard, as the provider of these models, does not control their usage by clients, complicating the balance between accuracy and fairness. Mastercard's primary responsibility is delivering accurate predictions, but this may conflict with promoting fairness, especially since the downstream application of predictions is uncertain.

Ensuring fairness in predictive models involves technical challenges, particularly in disentangling individual behaviors from demographic identities in spending patterns, aiming for consistent service quality without discrimination.

\begin{itemize} 
\item \textbf{Users/Clients:} Diverse needs necessitate representative data collection and feedback. Consider whether data and customer satisfaction feedback adequately represent all demographics. 
\item \textbf{Bank Officers/Customer Service Representatives:} Interface with clients, impacting data gathering and service levels. Assess their incentive structures and potential biases. 
\item \textbf{Senior Management/Executives:} Balance profit objectives with ethical, tailored financial products. Their understanding of fairness is crucial for strategic decisions.
\item \textbf{Shareholders/Investors:} Influence on prioritizing profit versus ethical product offerings. Evaluate their impact on decision-making. 
\item \textbf{General Public:} Public trust influences the success and adoption of financial services. Consider societal expectations around fairness.
\item \textbf{Regulators/Legislators:} Compliance with varying regulatory environments (e.g., US, EU) is essential. Determine the stringency of these regulations. 
\item \textbf{Developers/Data Scientists:} Conduct bias impact assessments and implement fairness metrics. Their influence on ethical AI practices is critical. 
\item \textbf{Consumer Advocacy Groups:} Advocate for marginalized communities, providing insights for fair practices. Assess their influence in decision-making. 
\item \textbf{Industry Associations/Standards Bodies:} Develop guidelines for fair and ethical AI in finance, shaping industry practices. 
\item \textbf{External Auditors/Ethics Boards:} Provide oversight and recommendations, ensuring fairness and accountability, becoming increasingly prominent as legislation advances. 
\end{itemize}

By addressing the diverse perspectives of these stakeholders, financial service providers can better ensure fairness, mitigate biases, and provide equitable access to financial products.
